Attention-based Encoder-Decoder Network for End-to-End Neural Speaker Diarization with Target Speaker Attractor

This paper proposes a novel Attention-based Encoder-Decoder network for End-to-End Neural speaker Diarization (AED-EEND). In AED-EEND system, we incorporate the target speaker enrollment information used in target speaker voice activity detection (TS-VAD) to calculate the attractor, which can mitigate the speaker permutation problem and facilitate easier model convergence. In the training process, we propose a teacher-forcing strategy to obtain the enrollment information using the ground-truth label. Furthermore, we propose three heuristic decoding methods to identify the enrollment area for each speaker during the evaluation process. Additionally, we enhance the attractor calculation network LSTM used in the end-to-end encoder-decoder based attractor calculation (EEND-EDA) system by incorporating an attention-based model. By utilizing such an attention-based attractor decoder, our proposed AED-EEND system outperforms both the EEND-EDA and TS-VAD systems with only 0.5s of enrollment data.

==> tables/enroll_thres_len_ablation.tex <==
\begin{table*}[ht!]
\footnotesize
\centering
\caption{\textbf{DER (\%) results comparison on different decoding methods with different enroll length and stop decoding length.} 
All the results are based on our 2-spk systems.
% and we evaluate the system on the 2-spk part of the simulation set and callhome part2 dataset.
\textbf{DEL}: differnt decoding length. \textbf{DSL}: different stop decoding length. The grey background is used to mark very poor results.
}
\begin{adjustbox}{width=.98\textwidth,center}
\begin{tabular}{c ccccccc ccccccc}
\toprule
\multirow{2}{*}{Decoding Method} & \multicolumn{7}{c}{DEL DER (\%) on Simu} & \multicolumn{7}{c}{DEL DER (\%) on Callhome}\\

\cmidrule(r){2-8} \cmidrule(r){9-15} 

& 0.1s & 0.5s & 1s & 2s & 3s & 5s & 10s & 0.1s &  0.5s & 1s & 2s & 3s & 5s & 10s \\
\hline

GT-Decode & 3.10 & 3.22 & 3.22 & 2.95 & 3.05  & 2.87  & 2.88  & 8.39 & 8.03  & 7.58 & 7.56 & 7.18  & 7.27  & 7.19  \\
Init-Decode & 5.18 & 3.14 & 3.14 & 6.34 & \grey 23.8 & \grey 67.1 & \grey 97.5 &  \grey 40.78 & 10.9 & 7.90 & 8.71 & \grey 15.1 & \grey 35.1 & \grey 86.1 \\
Rand-Decode & 3.36 & 3.13 & 3.18 & 6.73 & \grey 24.1 & \grey 67.2 & \grey 97.5 & 11.36 & 8.32  & 8.38 & 9.39 & \grey 16.0 & \grey 35.5 & \grey 86.1 \\
SC-Decode & 3.13 & 3.14 & 3.12 & 3.17 & 3.16  & 3.17  & 8.27  & 8.61 & 7.75  & 7.86 & 8.04 & 7.68  & 7.81  & 8.78 \\
\hline

% & 0.1s & 0.2s & 0.3s & 0.4s &  & & 0.1s & 0.2s & 0.3s & 0.4s &  &  \\
% \cmidrule(r){2-7} \cmidrule(r){8-13} 
% Mode-3 & 3.13 & 3.13 & 3.12 & 3.20 & - & - & 8.61 & 8.43 & 8.04 & 7.82 & - & - \\

\midrule
 & \multicolumn{7}{c}{DSL DER (\%) on Simu} & \multicolumn{7}{c}{DSL DER (\%) on Callhome}\\
\cmidrule(r){2-8} \cmidrule(r){9-15} 
& 0.5s & 0.8s & 1s & 1.5s & 2s & 2.5s & - & 0.5s & 0.8s & 1s & 1.5s & 2s & 2.5s & - \\
\hline
Init-Decode & 4.92 & 3.55 & 3.40 & 3.56 & 4.88 & \grey 10.03 & - & \grey 19.4 & 10.9 & 10.7 & 10.8 & 10.6 & 12.2 & - \\
Rand-Decode & 4.06 & 3.68 & 3.50 & 3.51 & 5.53 & \grey 10.85 & - & \grey 13.2 & 9.35  & 8.58  & 8.20  & 8.58  & 10.4 & - \\
SC-Decode & 3.98 & 3.55 & 3.25 & 3.53 & 6.59 & \grey 13.08 & - & \grey 13.0 & 8.28  & 8.34  & 8.47  & 9.36  & 11.5 & - \\
\hline
\bottomrule
\end{tabular}
\label{table:enroll_thres_len_ablation}
\end{adjustbox}
\end{table*}

==> tables/flexible_spk_num_callhome_more_res.tex <==
\begin{table}[ht!]
\footnotesize
\centering
\caption{\textbf{DER (\%) results on the CALLHOME dataset with flexible number of speakers.} For the line with $^*$ we use a different setup by directly training our model on the 1-4 speakers dataset for 100 epochs.
}
\begin{adjustbox}{width=.47\textwidth,center}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{6}{c}{spk\#}\\
\cmidrule(r){2-7}
 & 2 & 3 & 4 & 5 & 6 & all\\
 \hline
 x-vector clustering \cite{horiguchi2020end} & & & & &  \\
 \hspace{3pt} Estimated \#spk & 15.45 & 18.01 & 22.68 & 31.40 & 34.27 & 19.43 \\
 \hspace{3pt} Oracle \#spk & 8.93 & 19.01 & 24.48 & 32.14 & 34.95 & 18.98 \\

 EEND-EDA \cite{horiguchi2020end} & & & \\
 \hspace{3pt} Estimated \#spk & 8.50 & 13.24 & 21.46 & 33.16 & 40.29 & 15.29 \\
 \hspace{3pt} Oracle \#spk & 8.35 & 13.20 & 21.71 & 33.00 & 41.07 & 15.43 \\
 
 Ours & & & \\
 % from exp/2_spk/use_query_as_tgt/drop_spk_05_adapt_all/adapt_callhome_all_epoch_20-25/infer/callhome2_spkall/epochs80-90/spk_qty-1_spk_qty_thr10_mode_3
 \hspace{3pt} Estimated \#spk & 6.96 & 12.56 & \textbf{18.26} & 34.32 & 44.52 & 14.22 \\
 % from exp/2_spk/use_query_as_tgt/drop_spk_05_adapt_all/adapt_callhome_all_epoch_20-25/infer/callhome2_spkall/epochs90-100/spk_qty-1_spk_qty_thr-1_mode_3/score
 \hspace{3pt} Oracle \#spk & 6.79 & 12.36 & 19.84 & 32.42 & 37.08 & 14.00 \\

  Ours $^*$ & & & \\
 % from exp/all_spk/use_query_as_tgt/drop_spk_05_kaldi_4_process/adapt_callhome_all_epoch_95-100
 \hspace{3pt} Estimated \#spk & \textbf{6.62} & 11.97 & 18.85 & 31.69 & 36.10 & \textbf{13.52} \\
 % from exp/all_spk/use_query_as_tgt/drop_spk_05_kaldi_4_process/adapt_callhome_all_epoch_95-100/infer/callhome2_spkall/epochs50-55/spk_qty-1_spk_qty_thr-1_mode_3/score
 
 \hspace{3pt} Oracle \#spk & 7.72 & \textbf{11.59} & 19.28 & \textbf{30.89} & \textbf{33.31} & 13.69 \\


\bottomrule
\end{tabular}
\label{table:flexible_spk_num_callhome_res}
\end{adjustbox}
\end{table}

==> tables/flexible_spk_num_simu_more_res.tex <==
\begin{table}[ht!]
\footnotesize
\centering
\caption{\textbf{DER (\%) results on the simuation dataset with flexible number of speakers.}
}
\begin{adjustbox}{width=.36\textwidth,center}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{spk\#}\\
\cmidrule(r){2-5}
 & 1 & 2 & 3 & 4 \\
 \hline
 x-vector clustering \cite{horiguchi2020end} & & & \\
 \hspace{3pt} Estimated \#spk & 37.42 & 7.74 & 11.46 & 22.45 \\
 \hspace{3pt} Oracle \#spk & 1.67 & 28.77 & 31.78 & 35.76 \\

 EEND-EDA \cite{horiguchi2020end} & & & \\
 \hspace{3pt} Estimated \#spk & 0.39 & 4.33 & 8.94 & 13.76 \\
 \hspace{3pt} Oracle \#spk & 0.16 & 4.26 & 8.63 & 13.31 \\
 
 Ours & & & \\
 % from exp/2_spk/use_query_as_tgt/drop_spk_05_adapt_all/infer/swb_sre_cv_ns1n2n3n4_beta2n2n5n9_500/epochs20-25/spk_qty-1_spk_qty_thr10_mode_3/score
 \hspace{3pt} Estimated \#spk & 0.09 & 2.82 & 6.88 & 12.00 \\
 % from exp/2_spk/use_query_as_tgt/drop_spk_05_adapt_all//infer/swb_sre_cv_ns1n2n3n4_beta2n2n5n9_500/epochs20-25/spk_qty-1_spk_qty_thr-1_mode_3/score
 \hspace{3pt} Oracle \#spk & 0.09 & 2.82 & 6.57  & 11.50 \\

 Ours $^*$ & & & \\
 % from exp/all_spk/use_query_as_tgt/drop_spk_05_kaldi_4_process/infer/swb_sre_cv_ns1n2n3n4_beta2n2n5n9_500/epochs70-80/spk_qty-1_spk_qty_thr10_mode_3/score
 \hspace{3pt} Estimated \#spk & 0.07 & 2.88 & \textbf{6.01} & 10.51 \\
 % from exp/all_spk/use_query_as_tgt/drop_spk_05_kaldi_4_process/infer/swb_sre_cv_ns1n2n3n4_beta2n2n5n9_500/epochs45-50/spk_qty-1_spk_qty_thr-1_mode_3/score
 \hspace{3pt} Oracle \#spk & \textbf{0.07} & \textbf{2.79} & 6.19 & \textbf{9.81} \\

\bottomrule
\end{tabular}
\label{table:flexible_spk_num_simu_res}
\end{adjustbox}
\end{table}

==> tables/silence_single-spk_overlap_res.tex <==
\begin{table}[ht!]
\vspace{-5pt}
\footnotesize
\centering
\caption{\textbf{AED-EEND result (\%) on the non-speech, single-speaker speech and overlap speech prediction.} 
All the results are based on our 2-spk systems. For the evaluation metric with $^*$ superscript, we use the total duration of the utterance as the denominator to calculate the metric.
}
\begin{adjustbox}{width=.47\textwidth,center}
\begin{tabular}{c|cc|cc|cc}
\toprule
 \multirow{2}{*}{Dataset}  & \multicolumn{2}{c}{Non-Speech} & \multicolumn{2}{c}{Single-Speaker} & \multicolumn{2}{c}{Overlap}\\
\cline{2-7}
                    & FA & MISS & FA & MISS & FA & MISS \\
\hline
Simulation & 3.45 & 3.46 & 6.57 & 6.11 & 8.73 & 9.64 \\
  \textsc{CallHome} & 29.50 & 30.64 & 9.81 & 7.57 & 26.28 & 41.23 \\


\hline
 & FA$^*$ & MISS$^*$ & FA$^*$ & MISS$^*$ & FA$^*$ & MISS$^*$ \\
 \hline
 Simulation & 0.72 & 0.72 & 3.38 & 3.14 & 2.42 & 2.67 \\
  \textsc{CallHome} & 2.89 & 3.00 & 7.70 & 5.94 & 3.09 & 4.86 \\


\bottomrule
\end{tabular}
\label{table:silence_spk_overlap}
\end{adjustbox}
\vspace{-5pt}
\end{table}
